Smooth-Trajectron++: Augmenting the Trajectron++ behaviour prediction model with smooth attention

Understanding traffic participants' behaviour is crucial for predicting their future trajectories, aiding in developing safe and reliable planning systems for autonomous vehicles. Integrating cognitive processes and machine learning models has shown promise in other domains but is lacking in the trajectory forecasting of multiple traffic agents in large-scale autonomous driving datasets. This work investigates the state-of-the-art trajectory forecasting model Trajectron++ which we enhance by incorporating a smoothing term in its attention module. This attention mechanism mimics human attention inspired by cognitive science research indicating limits to attention switching. We evaluate the performance of the resulting Smooth-Trajectron++ model and compare it to the original model on various benchmarks, revealing the potential of incorporating insights from human cognition into trajectory prediction models.

==> Chapters/discussion.tex <==
\section{Discussion}\label{discussion}

% Difference Reported values T++ and Reproduced values

The results show a significant gap between reported and reproduced performance values in the \textit{Trajectron++} paper. The FDE and ADE exhibit notable differences, especially at shorter prediction horizons and for pedestrian-only predictions. The reproduced KDE-NLL values also diverge greatly from the reported values. Several factors may contribute to this deviation. First, the \emph{nuScenes} dataset might have been updated, affecting input data and model output. Secondly, hyper-parameters and model settings used by the authors could differ from those available on their GitHub page or online paper. Also, issues during the reproduction process, such as data downloading or package installation, could have occurred. Given the numerous potential causes and the scope of our study, further investigation was not pursued. However, it could be interesting for future research to reproduce the \textit{Trajectron++} paper on the \emph{nuScenes} dataset and compare their results both to those reported by the original paper and to the ones in this work.\\


% Reflect upon the results of Smooth-Attention on \emph{nuScenes} --> FDE,ADE consistently lower than reproduced, regardless of the beta value. This applies to pedestrian-only and vehicle only. KDE-NLL not better in beta-cases for pedestrian-only, but better for vehicle-only.

In the evaluation on the \emph{nuScenes} dataset, the \textit{Smooth-Trajectron++} consistently outperforms \textit{Trajectron++} in FDE and ADE. Regardless of the applied $\beta$-values, lower scores are achieved, with $\beta = 0.1$ usually performing the best. The addition of a smoothing term reduces both Final Displacement and Average Displacement errors for pedestrian and vehicle predictions. The smooth model also improves KDE-NLL for vehicle predictions compared to the reproduced version, indicating more accurate and reliable predictions. However, for pedestrian predictions, there is little difference between the Smooth-versions and the original model, with slightly worse KDE-NLL scores for \textit{Smooth-Trajectron++}. This suggests that predicting pedestrian behavior is more challenging than vehicle trajectories. The smoothing term might decrease the variety of predicted trajectory distributions, affecting the average and making it less similar to ground truth. Further research is needed to explore this hypothesis in other pedestrian-only scenarios. \\


In contrast to the perceived results from the \emph{nuScenes} dataset, the performed experiments on the benchmark offer a less straightforward answer to the question whether the general model's performance increases when adding a $\beta$-term to the loss function. Examining $\beta = 0.1$ as an example, which was often optimal in the \emph{nuScenes} dataset for FDE and ADE, there are instances of both performance improvement and decline. This variation may stem from differences in the benchmark datasets. While the \emph{nuScenes} dataset encompasses a wide range of sensor data with cars and pedestrians, the benchmark datasets mainly focus on cars (\emph{highD}), predominantly cars with a small percentage of pedestrians (rounD), and cars only in a driving simulator (L-GAP). The application of the smoothing term $\beta$ in the \textit{Smooth-Trajectron++} model relies on the attention module that compares different classes of traffic participants. In datasets where one class dominates, the smoothing term may not function as intended. Particularly in scenarios with only one other traffic participant, the output becomes similar to the base model due to the lack of comparative references. This is evident in the L-GAP dataset results. However, the consistent results across all smooth-versions and the base model in the L-GAP dataset validate the implementation of the Smooth-Attention. Based on these findings, it can be inferred that \textit{Smooth-Trajectron++} does not consistently outperform the base model ($T+$). Nevertheless, we argue that the overall performance is mostly comparable or occasionally better, suggesting that it does not hinder the general functionality of such a model. Further research using \textit{Smooth-Trajectron++} on datasets with a more balanced variety of traffic classes, similar to \emph{nuScenes}, is recommended to explore potential performance improvements.\\

%% Reflect back on big picture / introduction --> place essence of study in literature

Considering the wider implications of examining whether it is beneficial to incorporate insights from cognitive science into an existing machine-learning framework regarding trajectory prediction, we could say a few things. First, we showed that it is possible to reproduce the results of a state-of-the-art trajectory prediction model on a large-scale dataset with a practical approach in a time-span of several months. Secondly, we successfully implemented a cognitive-based novel idea, Smooth-Attention, without public-code availability and integrated it as a modification to \textit{Trajectron++}, which had its public-code available. Thirdly, we tested the model on various datasets to validate its performance and examine its generalizability. Broadly speaking, we show that it is possible to integrate an idea from cognitive science into a machine-learning framework and achieve increased performance on a large-scale autonomous driving dataset. Smooth-Attention seems to work better on such large-scale multi-agent datasets than on unbalanced datasets with few traffic agents. Also, the implementation of \textit{Smooth-Trajectron++} does not give convincingly consistent improvements in results on gap-acceptance scenarios using the benchmarking framework. However, the authors of the Smooth-Attention paper \cite{cao2022leveraging}  show an increase in FDE and ADE performance regarding the INTERACTION dataset \cite{zhan2019interaction}, which entails merging and roundabout scenarios. We advise to research the validity of these claims, no public-code available, and to perform experiments with \textit{Smooth-Trajectron} on the INTERACTION dataset to compare these results.

==> acknowledgments.tex <==
\section*{Acknowledgments}





==> figures/Table_ADE_at_col.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{highD} (rest) & {\scriptsize $4.861^{\pm 0.477}$} & {\scriptsize $4.198^{\pm 0.479}$} & {\scriptsize $5.895^{\pm 0.742}$} & {\scriptsize $5.121^{\pm 0.480}$} & {\scriptsize $4.590^{\pm 1.034}$} & {\scriptsize $\underline{4.120}^{\pm 0.159}$} & {\scriptsize $4.635^{\pm 0.409}$} & {\scriptsize $5.194^{\pm 1.244}$} & {\scriptsize $4.593^{\pm 0.387}$} & {\scriptsize $5.176^{\pm 0.624}$} & {\scriptsize $\underline{4.321}^{\pm 0.367}$} & {\scriptsize $6.214^{\pm 3.288}$} \\ 
& {\scriptsize $\underline{6.381}^{\hphantom{\pm 0.000}}$} & {\scriptsize $7.473^{\hphantom{\pm 0.000}}$} & {\scriptsize $7.295^{\hphantom{\pm 0.000}}$} & {\scriptsize $5.431^{\hphantom{\pm 0.000}}$} & {\scriptsize $6.434^{\hphantom{\pm 0.000}}$} & {\scriptsize $6.844^{\hphantom{\pm 0.000}}$} & {\scriptsize $7.319^{\hphantom{\pm 0.000}}$} & {\scriptsize $6.396^{\hphantom{\pm 0.000}}$} & {\scriptsize $6.825^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{5.371}^{\hphantom{\pm 0.000}}$} & {\scriptsize $6.598^{\hphantom{\pm 0.000}}$} & {\scriptsize $5.743^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> figures/Table_FDE_at_col.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{highD} (rest) & {\scriptsize $13.192^{\pm 1.884}$} & {\scriptsize $11.402^{\pm 1.697}$} & {\scriptsize $16.337^{\pm 2.082}$} & {\scriptsize $13.954^{\pm 1.107}$} & {\scriptsize $12.346^{\pm 3.286}$} & {\scriptsize $\underline{11.10}7^{\pm 0.464}$} & {\scriptsize $12.285^{\pm 1.593}$} & {\scriptsize $14.370^{\pm 3.614}$} & {\scriptsize $12.109^{\pm 1.024}$} & {\scriptsize $14.110^{\pm 1.482}$} & {\scriptsize $\underline{11.32}5^{\pm 1.023}$} & {\scriptsize $17.431^{\pm 10.003}$} \\ 
& {\scriptsize $\underline{16.56}2^{\hphantom{\pm 0.000}}$} & {\scriptsize $20.230^{\hphantom{\pm 0.000}}$} & {\scriptsize $19.131^{\hphantom{\pm 0.000}}$} & {\scriptsize $14.943^{\hphantom{\pm 0.000}}$} & {\scriptsize $17.325^{\hphantom{\pm 0.000}}$} & {\scriptsize $18.929^{\hphantom{\pm 0.000}}$} & {\scriptsize $19.694^{\hphantom{\pm 0.000}}$} & {\scriptsize $17.417^{\hphantom{\pm 0.000}}$} & {\scriptsize $18.364^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{14.45}5^{\hphantom{\pm 0.000}}$} & {\scriptsize $17.230^{\hphantom{\pm 0.000}}$} & {\scriptsize $16.427^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> figures/Table_accuracy_at_col.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{highD} & {\scriptsize $0.915^{\pm 0.001}$} & {\scriptsize $0.927^{\pm 0.003}$} & {\scriptsize $0.911^{\pm 0.005}$} & {\scriptsize $\underline{0.929}^{\pm 0.009}$} & {\scriptsize $0.915^{\pm 0.007}$} & {\scriptsize $\underline{0.929}^{\pm 0.007}$} & {\scriptsize $0.919^{\pm 0.005}$} & {\scriptsize $0.927^{\pm 0.005}$} & {\scriptsize $\underline{0.920}^{\pm 0.002}$} & {\scriptsize $0.928^{\pm 0.006}$} & {\scriptsize $0.915^{\pm 0.002}$} & {\scriptsize $0.927^{\pm 0.003}$} \\ 
& {\scriptsize $0.901^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.899^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.901^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.905}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.904}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.899^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.902^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.903^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.902^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.899^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.901^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.899^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{highD} (rest) & {\scriptsize $0.836^{\pm 0.042}$} & {\scriptsize $0.844^{\pm 0.021}$} & {\scriptsize $0.842^{\pm 0.039}$} & {\scriptsize $\underline{0.858}^{\pm 0.032}$} & {\scriptsize $\underline{0.860}^{\pm 0.018}$} & {\scriptsize $0.839^{\pm 0.024}$} & {\scriptsize $0.844^{\pm 0.021}$} & {\scriptsize $0.803^{\pm 0.026}$} & {\scriptsize $0.851^{\pm 0.020}$} & {\scriptsize $0.846^{\pm 0.013}$} & {\scriptsize $0.858^{\pm 0.018}$} & {\scriptsize $0.835^{\pm 0.033}$} \\ 
& {\scriptsize $0.701^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.704^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.718^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.704^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.725^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.773}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.732}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.734^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.697^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.665^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.708^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.708^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{rounD} & {\scriptsize $\underline{0.952}^{\pm 0.015}$} & {\scriptsize $0.984^{\pm 0.005}$} & {\scriptsize $\underline{0.952}^{\pm 0.015}$} & {\scriptsize $\underline{0.991}^{\pm 0.005}$} & {\scriptsize $\underline{0.952}^{\pm 0.015}$} & {\scriptsize $0.984^{\pm 0.005}$} & {\scriptsize $\underline{0.952}^{\pm 0.015}$} & {\scriptsize $\underline{0.991}^{\pm 0.005}$} & {\scriptsize $\underline{0.952}^{\pm 0.015}$} & {\scriptsize $0.987^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.952}^{\pm 0.015}$} & {\scriptsize $0.987^{\hphantom{\pm 0.000}}$} \\ 
& {\scriptsize $\underline{0.890}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.935^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.890}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.948^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.890}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.974}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.890}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.935^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.890}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.948^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.890}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.935^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{L-GAP} & {\scriptsize $\underline{0.889}^{\pm 0.016}$} & {\scriptsize $0.991^{\pm 0.003}$} & {\scriptsize $\underline{0.889}^{\pm 0.016}$} & {\scriptsize $0.986^{\pm 0.005}$} & {\scriptsize $\underline{0.889}^{\pm 0.016}$} & {\scriptsize $0.987^{\pm 0.008}$} & {\scriptsize $\underline{0.889}^{\pm 0.016}$} & {\scriptsize $0.986^{\pm 0.007}$} & {\scriptsize $\underline{0.889}^{\pm 0.016}$} & {\scriptsize $\underline{0.992}^{\pm 0.007}$} & {\scriptsize $\underline{0.889}^{\pm 0.016}$} & {\scriptsize $0.984^{\pm 0.007}$} \\ 
& {\scriptsize $\underline{0.590}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.904^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.590}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.910}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.590}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.904^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.590}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.910}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.590}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.904^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.590}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.910}^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> figures/Table_accuracy_at_start.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{highD} & {\scriptsize $0.871^{\pm 0.016}$} & {\scriptsize $0.885^{\pm 0.006}$} & {\scriptsize $0.874^{\pm 0.010}$} & {\scriptsize $0.887^{\pm 0.007}$} & {\scriptsize $\underline{0.881}^{\pm 0.010}$} & {\scriptsize $0.883^{\pm 0.015}$} & {\scriptsize $0.876^{\pm 0.006}$} & {\scriptsize $0.891^{\pm 0.007}$} & {\scriptsize $0.879^{\pm 0.007}$} & {\scriptsize $0.884^{\pm 0.010}$} & {\scriptsize $0.876^{\pm 0.013}$} & {\scriptsize $\underline{0.894}^{\pm 0.006}$} \\ 
& {\scriptsize $0.833^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.837^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.836^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.837^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.833^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.837^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.833^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.837^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.838^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.848}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.842}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.840^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{highD} (rest) & {\scriptsize $0.826^{\pm 0.047}$} & {\scriptsize $0.870^{\pm 0.010}$} & {\scriptsize $0.831^{\pm 0.041}$} & {\scriptsize $0.880^{\pm 0.037}$} & {\scriptsize $\underline{0.874}^{\pm 0.017}$} & {\scriptsize $\underline{0.904}^{\pm 0.015}$} & {\scriptsize $0.873^{\pm 0.034}$} & {\scriptsize $0.893^{\pm 0.012}$} & {\scriptsize $0.852^{\pm 0.036}$} & {\scriptsize $0.899^{\pm 0.031}$} & {\scriptsize $0.841^{\pm 0.056}$} & {\scriptsize $0.889^{\pm 0.019}$} \\ 
& {\scriptsize $0.604^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.684^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.581^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.711^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.604^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.729}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.590^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.703^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.588^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.695^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.661}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.679^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{rounD} & {\scriptsize $\underline{0.970}^{\pm 0.004}$} & {\scriptsize $0.983^{\pm 0.008}$} & {\scriptsize $0.969^{\pm 0.009}$} & {\scriptsize $0.981^{\pm 0.005}$} & {\scriptsize $0.964^{\pm 0.008}$} & {\scriptsize $\underline{0.984}^{\pm 0.007}$} & {\scriptsize $\underline{0.970}^{\pm 0.001}$} & {\scriptsize $0.982^{\pm 0.004}$} & {\scriptsize $0.969^{\pm 0.003}$} & {\scriptsize $0.982^{\pm 0.002}$} & {\scriptsize $0.967^{\pm 0.006}$} & {\scriptsize $0.978^{\pm 0.006}$} \\ 
& {\scriptsize $0.852^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.917^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.856}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.921}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.843^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.921}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.836^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.913^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.852^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.909^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.839^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.917^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{L-GAP} & {\scriptsize $\underline{0.688}^{\pm 0.022}$} & {\scriptsize $0.988^{\pm 0.006}$} & {\scriptsize $\underline{0.688}^{\pm 0.022}$} & {\scriptsize $0.985^{\pm 0.007}$} & {\scriptsize $\underline{0.688}^{\pm 0.022}$} & {\scriptsize $0.985^{\pm 0.010}$} & {\scriptsize $\underline{0.688}^{\pm 0.022}$} & {\scriptsize $0.988^{\pm 0.006}$} & {\scriptsize $\underline{0.688}^{\pm 0.022}$} & {\scriptsize $0.983^{\pm 0.011}$} & {\scriptsize $\underline{0.688}^{\pm 0.022}$} & {\scriptsize $\underline{0.989}^{\pm 0.005}$} \\ 
& {\scriptsize $\underline{0.505}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.920}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.505}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.914^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.505}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.914^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.505}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.907^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.505}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.907^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.505}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.920}^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> figures/Table_brake_at_crit.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{rounD} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} \\ 
& {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{1.000}^{\hphantom{\pm 0.000}}$} \\ 
\midrule 
\emph{L-GAP} & {\scriptsize $\underline{0.599}^{\pm 0.350}$} & {\scriptsize $\underline{0.497}^{\pm 0.497}$} & {\scriptsize $\underline{0.599}^{\pm 0.350}$} & {\scriptsize $\underline{0.497}^{\pm 0.497}$} & {\scriptsize $\underline{0.599}^{\pm 0.350}$} & {\scriptsize $\underline{0.497}^{\pm 0.497}$} & {\scriptsize $\underline{0.599}^{\pm 0.350}$} & {\scriptsize $0.494^{\pm 0.494}$} & {\scriptsize $\underline{0.599}^{\pm 0.350}$} & {\scriptsize $0.494^{\pm 0.494}$} & {\scriptsize $\underline{0.599}^{\pm 0.350}$} & {\scriptsize $\underline{0.497}^{\pm 0.497}$} \\ 
& {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.000}^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> figures/Table_roc_curve_at_col.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{highD} (rest) & {\scriptsize $0.899^{\pm 0.028}$} & {\scriptsize $0.916^{\pm 0.015}$} & {\scriptsize $0.885^{\pm 0.050}$} & {\scriptsize $\underline{0.924}^{\pm 0.016}$} & {\scriptsize $\underline{0.919}^{\pm 0.014}$} & {\scriptsize $0.917^{\pm 0.020}$} & {\scriptsize $0.910^{\pm 0.013}$} & {\scriptsize $0.874^{\pm 0.031}$} & {\scriptsize $0.901^{\pm 0.028}$} & {\scriptsize $0.918^{\pm 0.012}$} & {\scriptsize $0.914^{\pm 0.010}$} & {\scriptsize $0.898^{\pm 0.038}$} \\ 
& {\scriptsize $0.653^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.757^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.653^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.710^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.725^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.817}^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.763}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.779^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.624^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.708^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.633^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.715^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> figures/Table_roc_curve_at_start.tex <==
\begin{tabularx}{\textwidth}{X | CC | CC | CC | CC | CC | CC} 
\toprule 
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{12}{c}{\textbf{Models}} \\
& \multicolumn{2}{c}{$T_{\beta_1}$}& \multicolumn{2}{c}{$T_{\beta_2}$}& \multicolumn{2}{c}{$T_{\beta_3}$}& \multicolumn{2}{c}{$T_{\beta_4}$}& \multicolumn{2}{c}{$T_{\beta_5}$}& \multicolumn{2}{c}{$T+$} \\
\midrule 
\emph{highD} (rest) & {\scriptsize $0.889^{\pm 0.036}$} & {\scriptsize $0.915^{\pm 0.018}$} & {\scriptsize $0.893^{\pm 0.039}$} & {\scriptsize $0.925^{\pm 0.040}$} & {\scriptsize $\underline{0.933}^{\pm 0.014}$} & {\scriptsize $\underline{0.949}^{\pm 0.007}$} & {\scriptsize $0.922^{\pm 0.025}$} & {\scriptsize $0.925^{\pm 0.023}$} & {\scriptsize $0.890^{\pm 0.027}$} & {\scriptsize $0.936^{\pm 0.018}$} & {\scriptsize $0.884^{\pm 0.055}$} & {\scriptsize $0.930^{\pm 0.011}$} \\ 
& {\scriptsize $0.472^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.619^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.506^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.735^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.473^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.753}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.427^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.689^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.424^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.612^{\hphantom{\pm 0.000}}$} & {\scriptsize $\underline{0.659}^{\hphantom{\pm 0.000}}$} & {\scriptsize $0.700^{\hphantom{\pm 0.000}}$} \\ 
\bottomrule
\end{tabularx}


==> header.tex <==
\usepackage{standalone}
\usepackage[table,xcdraw]{xcolor} % added for table styles
\usepackage{booktabs}
\usepackage{cite}
\usepackage{hyperref}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{colormaps}
\usepackage{circuitikz}

\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    citecolor={blue},
    filecolor=magenta,      
    urlcolor=cyan,
    pdftitle={Overleaf Example},
    pdfpagemode=FullScreen,
    }
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
\usepackage{algorithm,algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage{biblatex}
\usepackage{tablefootnote}
\usepackage[caption=false, font=footnotesize]{subfig}
\usepackage{capt-of}  % <---
\usepackage{cuted}    % <===


\newcommand\xlabel[2][]{\phantomsection\def\@currentlabelname{#1}\label{#2}}

% \usepackage{algorithm} 
% \usepackage{algpseudocode} 

% \addbibresource{references.bib}

%\usepackage[
%    %backend=biber, 
%    natbib=true,
%    style=numeric,
%    sorting=none]{biblatex}

\usepackage{natbib}

%\addbibresource{references.bib}



==> title.tex <==
\begin{titlepage}

\begin{center}

%% Print the title
{\makeatletter
\largetitlestyle\fontsize{45}{45}\selectfont\@title
\makeatother}

%% Print the subtitle
{\makeatletter
\ifdefvoid{\@subtitle}{}{\titlestyle\fontsize{20}{20}\selectfont\@subtitle}
\makeatother}

\bigskip
\bigskip

by

\bigskip
\bigskip

%% Print the name of the author
{\makeatletter
\largetitlestyle\fontsize{25}{25}\selectfont\@author
\makeatother}

\bigskip
\bigskip

%% Print table with names and student numbers
\setlength\extrarowheight{2pt}
\begin{tabular}{lc}
    Student Name & Student Number \\\hline
    F.S.B. Westerhout & 4293940 \\
    %%(...) \\
\end{tabular}

\vfill

%% Print some more information at the bottom
\begin{tabular}{ll}
    Primary supervisor: & Arkady Zgonnikov \\
    Daily supervisor: & Julian Schumann \\
    Secondary supervisor: & Joost de Winter \\
    Institution: & Delft University of Technology \\
    Place: & Faculty of Cognitive Robotics, Delft \\
    Project Duration: & August, 2022 - May, 2023
\end{tabular}

\vspace{1cm}
\small{Cover Image: }

\end{center}

%% Insert the TU Delft logo at the bottom of the page
\begin{tikzpicture}[remember picture, overlay]
    \node at (current page.south)[anchor=south,inner sep=10pt]{
        \includegraphics{layout/tudelft/logo-black}
    };
\end{tikzpicture}

\end{titlepage}

